Many Episode Learning in a Modular Embodied Agent via End-to-End Interaction

In this work we give a case study of an embodied machine-learning (ML) powered agent that improves itself via interactions with crowd-workers. The agent consists of a set of modules, some of which are learned, and others heuristic. While the agent is not "end-to-end" in the ML sense, end-to-end interaction is a vital part of the agent's learning mechanism. We describe how the design of the agent works together with the design of multiple annotation interfaces to allow crowd-workers to assign credit to module errors from end-to-end interactions, and to label data for individual modules. Over multiple automated human-agent interaction, credit assignment, data annotation, and model re-training and re-deployment, rounds we demonstrate agent improvement.

==> droidlet.tex <==
\clearpage

\section{Design of Droidlet Agent}
\label{sec:dsl}

This appendix gives a high level description of Droidlet agent design.

Droidlet agent has a modular, heterogeneous architecture. It consists of 4 main components: controller, perception, memory and task, as shown in figure \ref{fig:droidlet_design}. 

\textbf{Task module} affects changes in the agent's world.

\textbf{Perception module} processes information from the world and stores them in memory.

\textbf{Memory module} is the nexus of information for all the other systems.

\textbf{Controller module} manages tasks, based on the state of memory.

All the components are designed to be swappable, meaning that they all can be used separately from the main agent, and can be replaced or combined as users see fit. Those modules can be a model learned via ML, a heuristic model via scripting, or a combined one via both.

For example, the NLU model which we presented experiment results on is a transformer based ML model. It is a part of the perception module and can be easily swapped out with  another model if it conforms to the perception API.



\begin{figure}
    \centering
    \includegraphics[width=16cm]{images/droidlet_design.png}
    \caption{Droidlet Agent Design}
    \label{fig:droidlet_design}
\end{figure}

==> review_6PGk.tex <==
CoLLAs 2022 Conference Paper95 Reviewer 6PGk
10 Apr 2022 (modified: 10 Apr 2022)CoLLAs 2022 Conference Paper95 Official ReviewReaders: Program Chairs, Paper95 Reviewers Submitted, Paper95 Authors

Summary: This paper describes a pipeline and interface to perform human-in-the-loop learning of an embodied agent operating in a simulated 3D voxel world. The pipeline includes multiple modular components, including natural language understanding, a high-level task controller, scripted atomic tasks, and a human interaction interface. Feedback/errors are provided via crowd-sourced human interactions, and routed between the different components via a decision tree of questions provided to the worker.

Strengths: - The paper is clearly written and easy to understand.
- The proposed pipeline is an interesting step towards a full human-in-the-loop interaction.

Weaknesses: - Scientific and technical contributions over previous work are unclear.
- Experiments do not provide much scientific insight from the perspective of learning algorithms
Overall Review: The paper is clearly written, and pursues an interesting direction in human-in-the-loop learning.

My main concerns are with regard to the technical contributions from the perspective of learning algorithms.

The paper focuses more on the details of the pipeline, human interface and UX; as such, it reads more as a design document than a scientific research paper. What are the key contributions and novelty of this method over previous work (such as Pratik et al 2021 and the various human-in-the-loop papers that are cited)? What are the key scientific/technical insights that would be useful for the community developing lifelong learning algorithms?
Relatedly, most of the experiments focus on UX and design of the interface to allow workers to provide feedback that can be routed to individual modules. This might be interesting from the perspective of UX, but it's not clear what scientific insights to draw that would be more broadly applicable to the community (perhaps this is just a case of the venue not being a good fit for the work)? Figure 4 details one learning experiment, but mainly compares the performance when training on the initial data, or on the aggregated data after multiple rounds of human feedback, rather than comparing different methods or baselines from the literature.

A few further comments and questions:
- While the title mentions "continual learning", this doesn't examine a continual learning setting, which has certain desiderata and assumptions (eg. a sequence of tasks, lack of access to previous tasks, focus on minimizing forgetting and maximizing transfer, etc). In any case, the experiments and related work aren't really relevant to continual learning, so perhaps "human-in-the-loop" learning would be a better name? Similarly, the "continually learned" model is just trained on all of the accumulated data, which does not represent a continual learning setting. See the below references for some survey and review works that may be useful.
- The intro argues that methods with modular components (some of them hand-engineered) can be more practical for real-world deployment, but there aren't any experiments or related work to support this. If this is intended to be one of the hypotheses/contributions of the paper, then I think it needs to be much better supported.
- It's not clear to me what the "re-biased model" is intended to show. Is there an intended use case for this? What is the purpose of training on the whole dataset, and then fine-tuning on the initial, limited dataset before the multiple rounds of feedback?

[1] Hadsell, Raia, et al. "Embracing change: Continual learning in deep neural networks." Trends in cognitive sciences 24.12 (2020): 1028-1040.
[2] Parisi, German I., et al. "Continual lifelong learning with neural networks: A review." Neural Networks 113 (2019): 54-71.
[3] Lesort, Timothée, et al. "Continual learning for robotics: Definition, framework, learning strategies, opportunities and challenges." Information fusion 58 (2020): 52-68.

Score: -2: Clear rejection

Modifications: I think the direction is an interesting one, and I encourage the authors to continue to make improvements to the work. In particular, I would like to see:
- A clearer statement of the contributions of this work over previous work in human-in-the-loop learning.
- A clearer exposition discussing the scientific and technical insights from this work that would be of relevance to the machine learning community.
- More detailed and quantitative experiments, including comparison to existing human-in-the-loop methods, to showcase and better understand the benefits of the proposed pipeline.

Confidence: 4: The reviewer is confident but not absolutely certain that the evaluation is correct


==> review_K84e.tex <==
CoLLAs 2022 Conference Paper95 Reviewer K84e
10 Apr 2022CoLLAs 2022 Conference Paper95 Official ReviewReaders: Program Chairs, Paper95 Reviewers Submitted, Paper95 Authors

Summary: This work developed a proof-of-concept system of human-in-the-loop interactive learning for an embodied agent in 3D simulation environments. The system enables human users to control the motions of a virtual character in the environment and to provide natural language instructions to command an autonomous agent to perform tasks. The behavior of the autonomous agent is implemented with a modular pipeline with heuristic-based perception and task modules and a learning-based NLU module to map the natural language instructions to programs in the agent's domain-specific language. The authors developed a learning pipeline to gather training data, annotating them with online annotators, and retraining and redeploying the model. The experiments demonstrated that the model performances increased over multiple rounds of human-agent interaction through re-training the NLU module. Further, they performed UI/UX studies to examine the impact of several design choices on the efficiency of data collection.

Strengths: + I really like the high-level framework this work introduced, which incorporates human feedback through human-agent interaction in an iterative and continual fashion. I believe that this framework opens the door to promising systems of continual learning of embodied agents.

+ The authors developed a proof-of-concept system that illustrated the feasibility of building an intuitive user interface that allows amateur annotators to interact with the learning agents through natural language and keyboard inputs. It offers a means to scale up this method with a large number of crowd workers who might not have the background knowledge of the underlying AI technologies or the system architecture.

+ Not only did the authors demonstrate the initial success of using growing sets of training data to improve the overall NLU performance over time, but they also performed HCI studies on the UI/UX designs of their system. These analyses shed new insight into how to streamline the process of human-agent interaction for future work.

Weaknesses: - Technical novelty: While this work claimed to address human-in-the-loop learning for embodied agents, a key difference the authors highlighted over prior work, such as Carlson et al. (2010) and Mitchell et al. (2018), it, in practice, focused on improving the NLU module in the modular agent model, with the "perception" and "task" (action) modules simplified away with handcrafted designs. Such simplifications rendered the technical contributions of this work rather incremental over prior work on human-in-the-loop (interactive) learning. Further, the use of manually engineered perceptual systems and task executors introduced information bottlenecks and led to compounding errors. I think the claim of "continual learning for embodied agents" could be much better supported if the authors demonstrated full-stack optimization of the agent performance, rather than one of the modules in the pipeline.

- Expensive annotations: Although this method enables human operators to interact with the agent via natural language, the data annotations can still be expensive, as it requires a set of highly skilled crowd workers to provide ground-truth parses for the natural language commands that are marked as an NLU error. This reliance on domain expertise could severely limit the scalability of the proposed method in reality.

- Baseline comparisons: This work only compared their model with two self-baselines that were trained/fine-tuned on different partitions of the aggregated dataset. Additional baselines on continual learning and interactive learning (as the authors reviewed in Sec. 3) should be added for stronger experimental validation. Further, based on the results in Figure 4(right), the continually-learned model seems to suffer significantly from catastrophic forgetting - the model trained on R_n has gradually decayed performances on T_0. It suggests that further investigations and model improvements should be done to mitigate the effect of catastrophic forgetting.

- The writing quality of this draft needs improvement:

1) Some terminologies used in the work are non-standard, without clear definitions. For example, what exactly is "end-to-end interaction" in the title? The abstract only stated that it is not end-to-end training in the ML sense, but it was not clearly explained in the main text. Further, I was also confused about the term "credit assignment", which is a common term in reinforcement learning. But I don't think that this is what the authors meant in this context, as there is no reward in this problem formulation. As far as I can see, the term "credit assignment" was only mentioned in the abstract and discussion (sec. 5) without a clear definition. The sentence "we aim to show that credit can be assigned to different components in a modular system" was also a bit out of context and difficult to understand.

2) The agent is built on top of the Droidlet agent (Pratik et al. 2021). This paper only includes sparse references to this prior work, rather than giving technical explanations of the Droidlet agent. As a result, the readers would have to read Pratik et al. 2021 to understand the designs of the modules. Therefore, I highly recommend the authors include a background section that provides a high-level overview of the Droidlet agent to make this paper more self-contained. In particular, more details should be included in Sec. 2.2 on how the NLU model is designed, rather than merely citing Srinet et al. 2020.

Overall Review: While this paper is well motivated with an ambitious, high-level objective, the execution of this work is still a bit immature. As described in the Weaknesses section, the model design, experimental validation, and the writing quality could be substantially improved. Therefore, the reviewer believes that this work could benefit a lot from another round of revision, thus recommending the rejection of this manuscript.

Score: -2: Clear rejection

Modifications: - Reduce the level of manual engineering in the design of perception and task execution modules, evaluate the overall agent performances in integration tests, and conduct error analysis through ablation studies of individual modules;
- Incorporate additional baselines and improve the model's ability to mitigate the effect of catastrophic forgetting;
- Improve the writing quality to make the technical approach clearly explained and self-contained, without excessive reliance on referencing prior publications;
- For the UI/UX experiments in Sec. 4.3, make it clear what the goals and hypotheses each experiment aimed to investigate and offer motivations why these factors are the most important ones to study.

Confidence: 4: The reviewer is confident but not absolutely certain that the evaluation is correct

==> review_oRuq.tex <==
CoLLAs 2022 Conference Paper95 Reviewer oRuq
11 Apr 2022CoLLAs 2022 Conference Paper95 Official ReviewReaders: Program Chairs, Paper95 Reviewers Submitted, Paper95 Authors

Summary: The paper presents a case study and blueprint for an agent that learns from end-to-end human interactions. The system is continual/life-long learning as data are collected, model retrained and redeployed and subsequent interactions generate more data to train the agent. The emphasis is on system design and particularly pipeline and UI design of the NLP commands that specify desired behavior.

Strengths: + One of the top strengths is that the paper is a much needed description of what challenges are faced by a system deployed in the real world that learns from human commands. The authors tackle a hairy problem and provide practical solution to several challenges, such as how to deal with crowd sourced workers, UI design choices, correcting errors in labeling etc. There is value in presenting this to the community as many of these practical challenges are typically ignored in literature.

+ The paper explains and provides data to support key design choices in pipeline and interface design. Again, practical considerations such as correcting annotations are analyzed and reported.

+ Some continual learning results are provided for the NLU model of the agent.

+ The description on how interactions with human workers are collected, validated and corrected (especially section 2.3) was presented very clearly and the system makes a lot of practical sense! 

+ Similarly, section 2.3.1 was excellent in specifying challenges faced with using human annotators and how to combat them.

+ Section 4.3.4 presents an interesting idea on how to incentivize human annotators working with embodied agents rather than static datasets.

Weaknesses: - In my opinion, a critical weakness of the paper is lack of clarity in presenting the core idea of the work. The abstract and introduction preview a holistic description of an embodied real world agent that learns from end-to-end interaction. The rest of the paper, especially the results section, focuses on the pipeline of the natural language command component of the agent alone. This expectation is not set until on the top part of page 5.

I will reserve the rest for the modifications section as I believe the weaknesses can be addressed in a rewritten version of the paper.
Overall Review: My rating is motivated mainly by the lack of clarity in the contributions of the work. I think the paper can be re-written to outline the main idea and the subsequent contributions to the community and become a valuable publication. Please see suggestions below.

Score: -2: Clear rejection

Modifications: My main feedback is to rewrite the leading sections (introduction, abstract, and setting) to clarify the focus of this work. There are important contributions but they are not stated explicitly and are currently getting lost in the noise. 

Some specific suggestions:
1. Include a paragraph in the introduction that clearly states the contributions of the work and the expected experiments to demonstrate the ideas.
2. The abstract suggests that some description of the agent architecture will be provided. There is some description of the NLU component, but I would suggest a section outlining briefly the whole of the architecture of the learning agent. There are some citations from which the agent is derived, but a clear description is warranted in a system design paper such as this.
3. Discussion on "Credit Assignment (C)" is lacking or unclear. Which component does this credit assignment refer to? Does it refer to credit assignment in the reinforcement learning sense or otherwise?
4. The introduction starts of discussing adapting pre-training networks, and there seems to be some results based on that in section 4.2, but it is unclear exactly which components of the agent are adapted with new data.
5. What is the effect of the embodied human agent described in the second paragraph of section 2.1.1? It is briefly mentioned here but it's effect on the interactions isn't clearly described.
6. What is "clarify when needed" referring to in section 2.1.2 second paragraph?
7. More explanation of figure 3 is needed.
8. In section 4.2, why is comparison being done on T0? What is the importance of the rebiasing baseline?

Confidence: 3: The reviewer is fairly confident that the evaluation is correct
